Generalized Uncertainty Principle and Quantum Gravity Phenomenology

The fundamental physical description of Nature is based on two mutually incompatible theories: Quantum Mechanics and General Relativity. Their unification in a theory of Quantum Gravity (QG) remains one of the main challenges of theoretical physics. Quantum Gravity Phenomenology (QGP) studies QG effects in low-energy systems. The basis of one such phenomenological model is the Generalized Uncertainty Principle (GUP), which is a modified Heisenberg uncertainty relation and predicts a deformed canon ical commutator. In this thesis, we compute Planck-scale corrections to angular momentum eigenvalues, the hydrogen atom spectrum, the Stern-Gerlach experiment, and the Clebsch-Gordan coefficients. We then rigorously analyze the GUP-perturbed harmonic oscillator and study new coherent and squeezed states. Furthermore, we introduce a scheme for increasing the sensitivity of optomechanical experiments for testing QG effects. Finally, we suggest future projects that may potentially test QG effects in the laboratory.

==> apx-commutator_LiLj.tex <==
\chapter{GUP modified angular momentum commutator}
\label{apx:commutator_LiLj}

Consider the commutator between two components of the angular momentum
\begin{equation}
	[L_i,L_j] = \epsilon_{imn} \epsilon_{irs} [x_m p_n, x_r p_s] = \epsilon_{imn} \epsilon_{irs} \{ x_m [ p_n, x_r ] p_s + x_r [x_m , p_s ] p_n \}~, \label{eqn:commutator_ang_mom}
\end{equation}
Using the GUP commutator in (\ref{eqn:GUP}), we obtain
\begin{multline}
		[L_i,L_j] = i \hbar \epsilon_{imn} \epsilon_{irs} \left \{ q_r p_n \left[ \delta_{ms} - \alpha \left(\delta_{ms} p + \frac{p_m p_s}{p} \right) + \alpha^2 (\delta_{ms} p^2 + 3 p_m p_s ) \right] + \right. \\
		\left. - q_m p_s \left[ \delta_{nr} - \alpha \left( \delta_{nr} p + \frac{p_n p_r}{p} \right) + \alpha^2 ( \delta_{nr} p^2 + 3 p_n p_r ) \right] \right\} = \\
		= i \hbar ( \epsilon_{mni} \epsilon_{mjr} x_r p_n - \epsilon_{nim} \epsilon_{nsj} x_m p_s ) ( 1 - \alpha p + \alpha^2 p^2) = \\
		 = i \hbar [ ( \delta_{ir} \delta_{nj} - \delta_{nr} \delta_{ij} ) x_r p_n - ( \delta_{is} \delta_{mj} - \delta_{ij} \delta_{ms} ) x_m p_s ] ( 1 - \alpha p + \alpha^2 p^2) 
		  = i \hbar \epsilon_{ijk} L_k ( 1 - \alpha p + \alpha^2 p^2)~,
\end{multline}

Consider now
\begin{equation}
	[L_i,p_l] = \epsilon_{ijk}(x_j p_k p_l - p_l x_j p_k) =
	i \hbar \epsilon_{ijk} \left[ \delta_{jl} p_k - \alpha \left( \delta_{jl} p p_k + \frac{p_j p_l p_k}{p} \right) + \alpha^2 (\delta_{jl} p^2 p_k + 3 p_j p_l p_k) \right]~,
\end{equation}
where we used the model in (\ref{eqn:GUP}).
We then have
\begin{equation}
	[L_i,p^2] = p_l[L_i,p_l] + [L_i,p_l]p_l = 0~. \label{eqn:commutator_Li_p2}
\end{equation}

To find the commutation relation between a component of the angular momentum and the magnitude of the linear momentum, we will first suppose that such a commutator depends only on the vector $\mathbf{p}$
\begin{equation}
	[L_i,p] = f(\mathbf{p})~.
\end{equation}
In this way, using the result just found we have
\begin{equation}
	0 = [L_i,p^2] = p[L_i,p] + [L_i,p]p = 2p[L_i,p]~,
\end{equation}
that means, for $p\not=0$,
\begin{equation}
	[L_i,p] = 0~. \label{eqn:commutator_Li_p}
\end{equation}

Finally we find
\begin{multline}
	[L_i^2,L_j] = L_i[L_i,L_j] + [L_i,L_j]L_i = i \hbar \epsilon_{ijk} [L_i L_k (1 - \alpha p + \alpha^2 p^2) + L_k (1 - \alpha p + \alpha^2 p^2) L_i] = \\
	= i \hbar \epsilon_{ijk} (L_i L_k + L_k L_i) (1 - \alpha p + \alpha^2 p^2)~,
\end{multline}
Summing over $i$ we find
\begin{equation}
	[L^2,L_j] = \sum_{i=1,2,3} [L_i^2,L_j] = 0~.
\end{equation}
